Transverse Field $\gamma$-Matrix Spin Chains

We introduce a simple lattice spin model that is written in terms of the well-known four-dimensional $\gamma$-matrix representation of the Clifford algebra. The local spins with a four-dimensional Hilbert space transform in a spinorial $(1/2,0) \oplus (0,1/2)$ representation of $SO(4)$, a symmetry of our model. When studied on a chain, and as a function of a transverse field tuning parameter, our model undergoes a quantum phase transition from a valence bond solid phase to a critical phase that is described by an $SU(2)_1$ WZW field theory.

==> saved.tex <==
\section{\label{append: gamma}Clifford algebra and the spin group}

We start from the Lie algebra of $\mathrm{SO}(4)$.
Recall the Lie algebra isomorphism $\mathfrak{so}(4)\cong \mathfrak{su}(2)\oplus\mathfrak{su}(2)$. 
The 6 abstract generators of $\mathfrak{so}(4)$ algebra are $J_{\m\n}=-J_{\n\m}$, where $\m,\n=1,2,3,4$, and they satisfy the standard rotation algebra
\begin{align}
    [J^{\m\n},J_{\r\s}]=i\d_{[\s}{}^{[\m}J^{\n]}{}_{\r]}\, .\label{eq: so4 algebra}
\end{align}
In Eq.(\ref{eq: so4 algebra}), $\d^{\m\n}$ was used to raise and lower the indices so that the resulting expression can be written more succinctly, with the help of the unnormalized antisymmetrization notation $A_{[\m} B_{\n]}:=A_\m B_\n-A_\n B_\m$.
By defining (repeated indices are implicitly summed over)
\begin{align}
   M^{\pm}_i:=-\frac{1}{2}\left(\frac{1}{2}\e_{ijk}J_{jk}\pm J_{i4}\right)\, ,~~~(i,j,k=1,2,3) \label{eq: M in terms of J}
\end{align}
we see that the $\mathfrak{so}(4)$ algebra splits into two mutually-commuting copies of $\mathfrak{su}(2)$:
\begin{align}
    [M^{+}_i,M^{-}_j]=0\, ,~~[M^{\pm}_i,M^{\pm}_j]=i\e_{ijk}M^{\pm}_k\, .
\end{align}

A choice of $\g$ matrices, or more precisely a choice of faithful matrix representation for the  generators of the Clifford algebra $Cl(4)$ as $4\times 4$ matrices, is the Weyl/chiral basis:
\begin{align}
    \g^j :=-\s^2\otimes\s^j=\begin{pmatrix} 0 & i\s^j\\
    -i\s^j & 0
    \end{pmatrix}\, ,\\
    \g^4 :=\s^1\otimes\s^0=\begin{pmatrix} 0 & \s^0\\
   \s^0 & 0
    \end{pmatrix}\, ,
\end{align}
where the $0$'s stand for $2\times 2$ zero matrices,  $\s^j$ are the usual Pauli matrices, and $\s^0$ is the $2\times 2$ unit matrix. 
The $\g$ matrices satisfy the Clifford algebra's defining relation
\begin{align}
    \{\g^\m,\g^\n\}=2\d^{\m\n}\, ,~~~~~(\m,\n=1,2,3,4)
\end{align}
where a unit matrix is understood at the right-hand side of the equation.
In this basis, the gamma matrices are Hermitian: $(\g^\m)\dg=\g^\m$.

We define $\g^5$ as the Hermitian matrix
\begin{align}
    \g^5:=-\g^1\g^2\g^3\g^4=\s^3\otimes\s^0=\begin{pmatrix} \s^0 & 0\\
    0 & -\s^0
    \end{pmatrix}\,,
\end{align}
and it satisfies
\begin{align}
    (\g^5)^2=1\, ,~~\{\g^5,\g^\m\}=0\, .
\end{align}
The $\mathfrak{so}(4)\simeq\mathfrak{spin}(4)$ generators are represented by the spin matrices
\begin{align}
    \s^{\m\n}:=\frac{i}{4}[\g^\m,\g^\n]\, ,
\end{align}
and they satisfy the Lie algebra relation Eq.(\ref{eq: so4 algebra}).
If we substitute $J^{\m\n}$ with $\s^{\m\n}$ in Eq.(\ref{eq: M in terms of J}), we obtain $M^{\pm}_i$ as the matrices
\begin{align}
    M^{+}_{i}=\begin{pmatrix}
        \s^i & 0\\
        0 & 0
    \end{pmatrix}\,,~~M^{-}_{i}=\begin{pmatrix}
        0 & 0\\
        0 & \s^i
    \end{pmatrix}\,.\label{eq: M+-}
\end{align}
Since $\g^\m$ are chosen to be Hermitian, the matrices $\s^{\m\n}$ and $M^{\pm}_i$ are also Hermitian. 
Thus, they define a unitary representation of the spin group $\mathrm{Spin}(4)$ through the exponential map.

Any irreducible representation (irrep) of the Lie algebra $\mathfrak{spin}(4)=\mathfrak{su}(2)\oplus \mathfrak{su}(2)$ or the Lie group $\mathrm{Spin}(4)=\mathrm{SU}(2)\times\mathrm{SU}(2)$ can be labeled by a pair of non-negative half-integers, $(s_+,s_-)$, where $s_{\pm}$ specifies the $\mathrm{SU}(2)$ irrep for the operators $\mathbf{M}^{\pm}$. 
E.g., in the Dirac spinor representation, the $\mathfrak{spin}(4)$ operators act on the inner product space $\mathbb{C}^4$ (with the standard inner product) via the matrices in Eq.(\ref{eq: M+-}). $\mathbb{C}^4$ splits into two isomorphic 2-dimensional subspaces (the left- and right-handed Weyl spinors) on which $\mathbf{M}^\pm$ acts irreducibly: the first subspace is denoted as $(\ha,0)$ because $M^+_i$ acts as $\s^i$ and $M^-_i$ acts trivially, while the opposite situation occurs in the second subspace labeled $(0,\ha)$. Therefore, the Dirac spinor representation is denoted by $(\ha,0)\oplus (0,\ha)$.

Although the Dirac spinor representation is reducible for $\mathfrak{spin}(4)$, it is a faithful irreducible representation of the Clifford algebra $Cl(4)$. 
Moreover, exponentiating the matrices from Eq.(\ref{eq: M+-}) will give us a faithful representation of $\mathrm{Spin}(4)$ as a matrix group.
The double cover $\r:\mathrm{Spin}(4)\rightarrow\mathrm{SO}(4)$ is given by the conjugation map: for any $g\in\mathrm{Spin}(4)$,
\begin{align}
    g \g^\m g^{-1}=R(\r(g))^\m{}_\n \g^\n \,,
\end{align}
where $R :\mathrm{SO}(4)\rightarrow \mathrm{GL}(4,\mathbb{R})$ is the fundamental representation.

If we add reflections to $\mathrm{Spin}(4)$, we get the $\mathrm{Pin}(4)$ group. In other words, $\mathrm{Pin}(4)$ is the semi-direct product of $\mathrm{Spin}(4)$ with 
\begin{align}
    \mathbb{Z}_2\simeq \{1,2\s^{15}\}\,.
\end{align}
Just as the spin group is the double cover of the special orthogonal group, $\mathrm{Pin}(4)$ is the double cover of the orthogonal group $\mathrm{O}(4)$.

The spinor representation is faithful for both $\mathrm{Spin}(4)$ and $\mathrm{Spin}(5)$, but it is only irreducible for $\mathrm{Spin}(5)$.

\section{TFGMM as a quantum spin-$\fracm{3}{2}$ model}
The TFGMM can be deemed as a spin model too, because all the operators $\g^\m,\g^5$ are polynomials of $\mathrm{SU}(2)$ generators in the spin-$\fracm{3}{2}$ representation.
\begin{align}
     \g^1&=\frac{3i}{8}(\hat{S}_{+}-\hat{S}_{-})+\frac{i}{2}\left(\hat{S}_{3}\hat{S}_{-}-\hat{S}_{+}\hat{S}_{3}\right)\nonumber\\
    &~~+\frac{i}{2}((\hat{S}_{3})^2\hat{S}_{-}-\hat{S}_{+}(\hat{S}_{3})^2)+\frac{i}{6}((\hat{S}_{+})^3-(\hat{S}_{-})^3)\\
    \g^2&=-\frac{3}{8}(\hat{S}_{+}+\hat{S}_{-})+\frac{1}{2}\left(\hat{S}_{3}\hat{S}_{-}+\hat{S}_{+}\hat{S}_{3}\right)\nonumber\\
    &~~+\frac{1}{2}((\hat{S}_{3})^2\hat{S}_{-}+\hat{S}_{+}(\hat{S}_{3})^2)+\frac{1}{6}((\hat{S}_{+})^3+(\hat{S}_{-})^3)\\
    \g^3&=\frac{i}{\sqrt{3}}\left[(\hat{S}_{+})^2-(\hat{S}_{-})^2+(\hat{S}_{+})^2\hat{S}_{3}-\hat{S}_{3}(\hat{S}_{-})^2\right]\\
    \g^4&=\frac{1}{2\sqrt{3}}(\hat{S}_{+})^2+\frac{1}{2\sqrt{3}}(\hat{S}_{-})^2\\
    \g^5&=-\frac{2}{3}(\hat{S}_3)^3+\frac{13}{6}\hat{S}_3\,,
\end{align}
where the spin-$\fracm{3}{2}$ operators are defined by
\begin{align}
    \hat{S}_1=\ha\begin{pmatrix}
     0 & \sqrt{3} & 0 & 0\\
     \sqrt{3} & 0 & 2 & 0\\
     0 & 2 & 0 & \sqrt{3}\\
     0 & 0 & \sqrt{3} & 0
    \end{pmatrix}\,,\\
    \hat{S}_2=\frac{i}{2}\begin{pmatrix}
     0 & -\sqrt{3} & 0 & 0\\
    \sqrt{3} & 0 & -2 & 0\\
     0 & 2 & 0 & -\sqrt{3}\\
     0 & 0 &\sqrt{3} & 0
    \end{pmatrix}\,,\\
    \hat{S}_{3}=\ha\begin{pmatrix}
        3 & 0 & 0 & 0\\
        0 & 1 & 0 & 0\\
        0 & 0 & -1 & 0\\
        0 & 0 & 0 & -3
    \end{pmatrix}\,,
\end{align}
and $\hat{S}_{\pm}=\hat{S}_1\pm i \hat{S}_{2}$.

There exists a local Hilbert space basis in which the spin operators $\hat{S}_i$ span a Lie-subalgebra of the Lie algebra $\mathfrak{spin}(5)$ generated by $\s^{\m\n}$ and $\s^{5\m}$, but there is no basis in which they form a subalgebra of $\mathfrak{spin}(4)$ generated by $\s^{\m\n}$. 

Conceptually, there is no advantage of treating the TFGMM as a spin-$\fracm{3}{2}$ system; writing the TFGMM in terms of $\hat{S}_i$ will result in a cumbersome expression, hiding the symmetries of the theory.
Additionally, TFGMM does not possess the $\mathrm{SU}(2)$ symmetry generated by $\hat{S}_i$.

\section{\label{append: proj sym}Projective symmetry groups}
Each of the global internal symmetry groups $G_m$ in Table (\ref{table: symmetries}) has a faithful linear representation on the total Hilbert space $\mathscr{H}\simeq \mathbb{C}^{4^L}$.
However, the true symmetry group of the quantum system acts faithfully on the projective Hilbert space, so a mathematician would prefer study the projective symmetry groups: if a symmetry group $G$ acts linearly on a vector space $V$, then its projective symmetry group $PG$ is defined by 
\begin{align}
    PG=G/\{g\in G~|~\exists c\in \mathbb{C}~s.t. ~gv=c v~\forall v\in V\}\,,
\end{align}
i.e., it is $G$ defined up to scaling transformations. 
Note that the scaling transformations form a subgroup of $Z(G)$, the center of the group. For example, for any nontrivial element $g\in G_1$, there are at least two orthogonal states $v_{\pm}\in \mathscr{H}$ such that $gv_{\pm}=\pm v_{\pm}$, so
\begin{align}
    PG_1=G_1=\mathbb{Z}_2\times \mathbb{Z}_2\times \mathbb{Z}_2\,.
\end{align}
Since we restrict to even $L$, the eigenvalues of $\S^{12}$ will include $0$ and some nonzero values, so the only scalar transformation inside $G_2=\mathrm{U}(1)$ is the identity:
\begin{align}
    PG_2=G_2=\mathrm{Spin}(2)=\mathrm{U}(1)\,.
\end{align}
Similarly, for even $L$ there exist spin singlet states and non-singlet states for $\mathrm{SU}(2)$, so
\begin{align}
    PG_3=G_3=\mathrm{Spin}(3)=\mathrm{SU}(2)\,,\\
    PG_4=G_4=\mathrm{Spin}(4)=\mathrm{SU}(2)\times \mathrm{SU}(2)\,.
\end{align}
Thus, in all cases of TFGMM with even $L$, the global internal symmetry groups are exactly the projective symmetry groups.

For odd $L$, the projective symmetry group will in general act on the Hilbert space via a projective representation which is different from the linear representation of the original $G_m$. 
E.g., if $L=1$, then $PG_2=\mathrm{Spin}(2)/\{\pm I\}$. Although $PG_2$ is still isomorphic to $G_2=\mathrm{U}(1)$ as an abstract group, the group representation on the Hilbert space has changed.
The original symmetry group $\mathrm{U}(1)$ acts as such: the angle $\q\in [0,2\p)$ corresponds to the Hilbert space operator
\begin{align}
    g(\q)=e^{2i\q \S^{12}}\,,
\end{align}
and the group operation between any $\q_1,\q_2\in[0,2\p)$ is defined as summation mod $2\p$. 
To obtain $PG_2$, we impose the following equivalence relation:
\begin{align}
    g(\q)\sim g(\q+\p)\,.
\end{align}
Thus, the elements of $PG_2$ is parameterized by $\q\in [0,\p)$, where the group operation is summation mod $\p$.
Another example: if $L=1$, then $PG_3\simeq\mathrm{Spin}(3)/\{\pm I\}\simeq\mathrm{SO}(3)$ which is not isomorphic to $G_3=\mathrm{SU}(2)$ as a group.

\section{\label{sec: m=1} General $m$ TFGMM}
We define the $d=1$ transverse-field $\g$ matrix model (TFGMM) as the following families of Hamiltonians:
\begin{align}
    \hat{H}_m(\l)=\sum_{j=1}^{L}\left[\l\sum_{\m=1}^{m}\g^\m_j\g^\m_{j+1}+\sqrt{1-\l^2}\g^5_j\right]\,,\label{eq: TFGMM definition}
\end{align}
where $m=1,2,3,4,5$ and $-1\le \l \le 1$.  The $\g^5$ matrix is defined as $\g^5=-\g^1\g^2\g^3\g^4$.
When $\a=0$, we call $\hat{H}_{m}(\pm,0,L)$ as a $\g$ matrix model (GMM); for general $\a$, we call $\hat{H}_m(\pm,\a,L)$ as a TFGMM.
\subsection{$m=1$ and $m=2$}

It turns out that the $m<5$ TFGMM spectra are symmetrical under the $\mathbb{Z}_2\times\mathbb{Z}_2$ transformations, whereas the $m=5$ TFGMM spectrum is only invariant under $\car_{51}$ but not under $\car_{5}^{odd}$.
Hence, the sign of the transverse term doesn't matter; this fact justifies our usage of the transverse field parameter $\sqrt{1-\b^2}$.
Moreover, for $m<5$, we only need to consider the range $0\le \b\le 1$, whereas for $m=5$ we need the full range $-1\le \b \le 1$.

Let $\{b_j\}$ denote an arbitrary $L$-bit binary sequence. For each choice of such sequence, we can define a Hilbert subspace spanned by products of local states of the form $\bigotimes_{j}\ket{a_j,b_j}_j$, where $a_j=1,2$, and
\begin{align}
    \ket{1,+}=\begin{pmatrix}
        0 \\ 1 \\ 0 \\ 0
    \end{pmatrix}\,,~~\ket{2,+}=\begin{pmatrix}
        0 \\ 0 \\ 1 \\ 0
    \end{pmatrix}\,,\\
    \ket{1,-}=\begin{pmatrix}
        1 \\ 0 \\ 0 \\ 0
    \end{pmatrix}\,,~~\ket{2,-}=\begin{pmatrix}
        0 \\ 0 \\ 0 \\ 1
    \end{pmatrix}\,.
\end{align}
This basis allows us to split the total Hilbert space into $2^L$ many subspaces (one for each sequence $\{b_j\}$), each of dimension $2^L$. Then one can show that $\hat{H}_1$ and $\hat{H}_2$ act frustrated spin chains when restricted on these subspaces.

The $m=1$ TFGMM is equivalent to the direct sum of $2^L$ copies of the same Ising chain, each acting on only one Hilbert subspace associated with some $\{b_j\}$:
\begin{align}
     \hat{H}_{\text{Ising}}(\pm,\a,L)=\sum_{j}\left[\pm\sqrt{1-\a^2}\s^2_j \s^2_{j+1}+\a\s^3_j\right]\,.
\end{align}
Similarly, the $m=2$ TFGMM is the direct sum of $2^L$ copies of frustrated Heisenberg spin-$\ha$ chains:
\begin{align}
    \hat{H}_2(\pm,\a,L)&=\bigoplus_{\{b_j\}}\hat{H}_2[\{b_j\}]\,,\\
    \hat{H}_2[\{b_j\}]=&\pm\sqrt{1-\a^2}\sum_j (-1)^{b_j+b_{j+1}}\s^1_j\s^1_{j+1}\nonumber\\
    &\pm\sqrt{1-\a^2}\sum_j \s^2_j \s^2_{j+1}+\a\sum_j \s^3_j \,.\label{eq: m=2 spin chain}
\end{align}

As mentioned previously in \ref{subsec: gauge}, these two theories have spatially local symmetries. Our choice of basis $\ket{a,b_j}$ is compatible with these symmetries in that the symmetries do not mix states coming from subspaces defined by different sequences $\{b_j\}$.

\subsection{$m=3$}
When $|\b|=1$, there is a $\mathrm{U}(1)$ spatially local symmetry generated by $\s^{45}$. When $|\b| <1$, there is no local symmetry. There is an $\mathrm{SU}(2)$ global symmetry generated by $\S^{23},\S^{31},\S^{21}$. The spin quantum numbers corresponding to this global symmetry can be used to label the energy eigenstates. 

Now we solve the special case of $|\b|=1$, which does not involve any transverse term. 
We can choose the $\mathrm{U}(1)$ local gauge charge to be $\pm \ha$ at each site.
Each such choice is specified by the $L$-bit binary sequence $\{b_j\}$, where the spatially local symmetry charge at site $j$ is $(-1)^{b_j}\ha$.
At each site, the local Hilbert space corresponding to $b_j$ is spanned by the 2 eigenvectors of $(\s^{54})_j$ with eigenvalue $(-1)^{b_j}\ha$:
\begin{align}
    \ket{\pm,1}=\frac{1}{\sqrt{2}}\begin{pmatrix}
      \pm i \\ 0 \\ 1 \\ 0
    \end{pmatrix}\,,~~\ket{\pm,2}=\frac{1}{\sqrt{2}}\begin{pmatrix}
        0 \\ \pm i \\ 0 \\ 1
    \end{pmatrix}\,.
\end{align}
The global symmetry generators act on the local subspace at site $j$ by
\begin{align}
    \S^{ik}\ket{\pm,a}_j=-\frac{1}{2}\e^{ikl}(\s^l)_{ab}\ket{\pm, b}_j\,,
\end{align}
for $i,k,l\in\{1,2,3\}$.


Restricted to this local subspace, the $\g$ matrices that appear in $\hat{H}_3$ become 
\begin{align}
    (\g^i)_j\rightarrow (-1)^{b_j}(\s^i)_j ~~~~ i=1,2,3\,.
\end{align}
Thus, the theory is the direct sum
\begin{align}
    \hat{H}_3(\pm,0,L)=\bigoplus_{\{b_j\}}\hat{H}_3[\{b_j\}]\,,
\end{align}
where $\hat{H}_3[\{b_j\}]$ first projects to the Hilbert subspace corresponding to the sequence $\{b_j\}$, then act as
\begin{align}
    \hat{H}_3[\{b_j\}]=\pm\sum_{j}(-1)^{b_j+b_{j+1}}(\s^i)_{j}(\s^i)_{j+1}\,.
\end{align}

% A few observations for the $m=3$, $|\b|=1$ theory: 
% \begin{enumerate}
%     \item Each energy level has an even degeneracy. This is because $\hat{H}_3[\{b_j\}]=\hat{H}_3[\{b'_j\}]$ given that 
%     \begin{align}
%         b_j=b'_j+1 ~~(\text{mod} 2)~~~\forall j=1,\cdots,L\,.
%     \end{align}
%     \item The ground state energy of the $m=3$ GMM is exactly the ground state energy of the antiferromagnetic Heisenberg spin-$\ha$ chain. Such a spin chain is described by $b_j=constant$ for all $j=1,2,\cdots, L$ in our Hamiltonian. Since the constant can only take two values (either 0 or 1), the ground state is doubly degenerate, consistent with the previous point.
%     \item For any integer $L>2$ and any choice of the $L$-bit binary sequence $\{b_j\}$, there are an even number of ferromagnetic bonds (FB) in $\hat{H}_3[\{b_j\}]$, i.e. bonds that have coefficient $-1$.
%     \item Generally, the less frustration (number of domain walls) a spin chain has, the lower its ground state energy. 
%     \item For those Hamiltonians with exactly two ferromagnetic bonds (FB), if there are an even number of antiferromagnetic bonds (AFB) between the FBs, then the ground state is 3-fold degenerate; if there are an odd number of AFBs between the two FBs, then the ground state is unique.
%     \item After the antiferromagnetic Heisenberg chain, the Hamiltonians $\hat{H}_3[\{b_j\}]$ with the next lowest ground state have exactly two ferromagnetic bonds that are separated from each other by exactly one AFB.
% \end{enumerate}
% For instance, for $L=4$, the first excited states are ground states for the spin chain with bond coefficients $(1,-1,1,-1)$ and $(-1,1,-1,1)$. Therefore, the first excited energy level has a degeneracy of $2\times 2=4$.
% For $L=6$, the first excited states are ground states for the spin chain with bond coefficients $(-1,1,-1,1,1,1)$, $(1,-1,1,-1,1,1)$, $(1,1,-1,1,-1,1)$, $(1,1,1,-1,1,-1)$, $(-1,1,1,1,-1,1)$, and $(1,-1,1,1,1,-1)$. Therefore, the first excited energy level has a degeneracy of $2\times 6=12$.
% If this argument is true in general, then we expect the first excited state to be $2N$-fold degenerate for any even $L>2$. Indeed, this is what we observe for small system sizes: it has been verified up to $L=8$.

% The method explained in this subsection do not work for $m=4$, since $\g^4$ mixes the $\pm$ subspaces:
% \begin{align}
%     \g^4\ket{\pm,a}=\pm i \ket{\mp,a}\,.
% \end{align}

% Finally, we note that there is a way to understand why the sign of the hopping term for the $m=3$ TFGMM doesn't matter. 
% We have just seen that the Hamiltonian is the direct sum of all possible $\mathrm{O}(3)$-symmetric Heisenberg spin-$\ha$ chains, including the antiferromagnetic chain and the ferromagnetic chain.
% Multiplying the hopping terms by a sign may map one spin chain to another, but the new Hamiltonian is still the same direct sum of all possible Heisenberg spin chains.

The $\a\ne 0$ case is much trickier than the $\a=0$ case.
The local invariant subspace for all of $\g^1_j,\g^2_j,\g^3_j,\g^5_j$ is simply the 4-dimensional local Hilbert space because
\begin{align}
     \g^5\ket{\pm,a}=- \ket{\mp,a}\,,
\end{align}
so we cannot decompose $\hat{H}_3(\b,L)$ into a direct sum.
Moreover, there is no spatially local symmetry.

% We show that there is an interesting duality: there is an equivalent theory in which the on-site interaction term corresponds to the TFGMM's hopping term, and the hopping term corresponds to the TFGMM's on-site interaction terms. 
% Consider an array of $2^L$ many Heisenberg spin-$\ha$ chains, where each chain is seen as a ``site". Each such site has a unique site index $I$, ranging from $0$ to $2^L-1$. We choose to represent $I$ in binary digits: $I=0,1,10,11,100$, etc. In other words, the set of all index $I$ is isomorphic to the set of all $L$-bit binary sequences $\{b_j\}$. 
% Moreover, we say $I'$ is a neighbor of $I\sim\{b_j\}$ whenever $I'-I\in (-1)^{b_k} 2^{k-1}$ for some positive integer $k$.
% Thus, each site has exactly $L$ neighbors.
% Now we specify that the spin chain at site $\{b_j\}$ is exactly $\hat{H}_{3}[\{b_j\}]$ as described in the previous subsection.
% Thus, the hopping terms $\sum_{\m=1}^{3}\g^\m_j\g^\m_{j+1}$ from the original Hamiltonian $\hat{H}_3$ now correspond to on-site terms in the new perspective.
% Similarly, the on-site interaction term $\g^5_j $ from the original Hamiltonian now becomes a hopping term. 
% At the site $I\sim \{b_j\}$, the local Hilbert space is $2^L$-dimensional and is spanned by tensor product states of the form $\ket{I;\{a_j\}}$, where $a_j=1,2$. Then $\g^5_k$ acts by
% \begin{align}
%     \g^5_k\ket{I;\{a_j\}}=-\ket{I+(-1)^{b_k}2^{k-1};\{a_j\}}\,.
% \end{align}
% By our definition of neighboring spin chains, the interaction term $\g^5_k$ which is on-site in the original Hamiltonian can now be seen as a nearest-neighbor hopping term.
% In fact, it is like the translation operators in an $L$-dimensional space.
% There are important differences between these two perspectives. In the original view, the Hilbert space is a tensor product of local Hilbert spaces, whereas now the Hilbert space is a direct sum of local Hilbert spaces. Moreover, originally the on-site terms are position-independent, but now the on-site terms are position-dependent. 
% We will not go further with this analogy.

The 2-site problem has energy eigenstates of the form $\ket{E,s,m_s}$, which are either spin singlets or triplets. The triplets ($s=1$) have energies  $E=\pm 2$ and $E=\pm 2\sqrt{1-\a^2}$. 
The spin singlets ($s=0$) have energies $E=\pm 6\sqrt{1-\a^2}$ and $E=\pm 2\sqrt{9-8\a^2}$. 


The effective Hamiltonian acting on the nearly $2^L$-fold degenerate ground state at the regime of $\a=\sqrt{1-\e^2}$ where $0\le \e \ll 1$ (in the fermionic perspective, this is at half-filling) is
\begin{align}
    \hat{H}_{3,\text{eff}}=&L\left(-1-\frac{1}{4}\e^2+\frac{11}{64}\e^4\right)\nonumber\\
    &+\e^2\left(\ha-\frac{7}{16}\e^2\right)\sum_{j}\s^i_j\s^i_{j+1}\nonumber\\
    &+\frac{\e^4}{4}\sum_{j}\s^i_j\s^i_{j+2}+\co(\e^5)\,.
\end{align}
which is an antiferromagnetic spin-$\ha$ $J_1-J_2$ model up to the 4th order.
Note that this expression is valid only for $L>4$. For $L<4$, it is slightly different, but since these simple cases can be studied exactly without using any perturbation theory, we don't bother to discuss them.
% The fluid-dimer transition of the $J_1-J_2$ model happens at $\frac{J_2}{J_1}\approx 0.24$, which, according to the effective Hamiltonian, corresponds to $\a\approx \pm 0.81$ or $\b\approx \pm 0.58$. The Majumdar-Ghosh model corresponds to $\a\approx \pm 0.68$ or $\b\approx \pm 0.73$. 

% In Fig.\ref{fig: PBC L=4 m=3 exact spectrum}, first focus on the green dashed curve starting from $E-E_0\approx 1$ at $\a=0$ that eventually goes to $E-E_0=0$ at $\a=1$, and the golden solid curve that starts from $E-E_0\approx 2.4$ at $\a=0$ and ends at $E-E_0=0$ at $\a=1$. The green curve is a singlet, while the golden curve is a triplet, and both of them have momentum $k=\p$. They intersect at $\sqrt{\frac{2}{3}}\approx 0.816497$.
% These two curves are also present in the $m=4$ case, and they intersect at almost the same point, as we will see later. 

% Next, we note that the GS is almost doubly degenerate when $\a\ll 1$. In fact, the energy gap between those two singlet states grows as $\a^L$ to the lowest order. These two singlets also share the same momentum eigenvalue: for $L=4$, it is $k=0$.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Picture/PBC L=4 m=3 exact spectrum.png}
%     \caption{The lowest few energy levels measured from the ground state, shown with their spin irrep. When $\a=0$, the first excited state has degeneracy 4. When the transverse field is switched on, two of them remain degenerate. All these 4 states are spin singlets.}
%     \label{fig: PBC L=4 m=3 exact spectrum}
% \end{figure}

% \textcolor{red}{Conjectures/Observations:} 
% \begin{enumerate}
%     \item The energy splitting in the approximately doubly degenerate ground state goes like $\a^L$ to the lowest order.
%     \item At $\a=0$, the 1st excited energy has a degeneracy of $2N$, for any $L>4$.
%     % \item The energy gap at $\a=0$ will close up in the thermodynamic limit.
%     \item For any $L>4$, at $\a=0$, the 2nd excited energy has a degeneracy of $3N$ if $L\in 4\mathbb{Z}+2$, or $L$ if $L\in 4\mathbb{Z}$.
% \end{enumerate}
% The first 2 points have been verified for small system sizes and can be explained easily. When $\a=0$, the ground states are exactly 2 copies of the ground state of the ferromagnetic Heisenberg chain, denoted as $\ket{\j_+}$ and $\ket{\j_-}$. The state $\ket{\j_{+}}$ lives in the subspace defined by the constant sequence $\{0,0,0,\cdots,0\}$, while the state $\ket{\j_{-}}$ lives in the subspace defined by the constant sequence $\{1,1,1,\cdots,1\}$.
% Together, these two states form a 2-dimensional degenerate energy level.
% Now we study what happens when the interaction term $\hat{V}_{int}=\a\sum_j(\g^5)_j$ is introduced.
% For each $j$, the operator $\g^5_j$ simply maps $\ket{\pm,a}$ to $-\ket{\mp,a}$ within the local Hilbert space.
% However, we also know $\ket{\j_+}$ can only be mapped into $\ket{\j_-}$ by simultaneously changing all its $b_j=0$ to $b'_j=1$, which is only possible by applying 
% $(\hat{V}_{int})^L\sim \a^L\prod_j (\g^5)_j$.
% Although $V^2$ can map from $\ket{\j_+}$ or $\ket{\j_-}$ back to itself, it cannot map between them.
% Moreover, $\g^5$ acts in the same way on both $\ket{\pm,a}$. Thus, the splitting of the ground state cannot be contributed by $V^k$ for any $1\le k <L$; the lowest order contribution to the spitting between these two approximately degenerate levels is of order $\a^L$.
% One consequence of this fact is that in the thermodynamic limit $L\rightarrow \infty$, there is an interval $I=[0,\a_c]$ such that whenever $\a\in I$ the ground state is doubly degenerate. Even for finite system size and any $\a$, these approximately degenerate ground states are exact eigenstates of the idempotent operator $\car_{5}$ with eigenvalues $\pm 1$.

% A similar argument can be applied to describe the energy splitting of the 1st excited state. E.g., take $L=6$. One of the 1st excited states is described by the sequence $(1,1,0,0,0,0)$, and we want to find the minimum number of flips (each flip can change a $0$ to $1$ or vice versa, at a single site) needed to transform it to $(0,1,1,0,0,0)$ or $(0,0,1,1,0,0)$, etc. It is clear that this number is $2$ for large enough $L$, but for small $L$ we could have $\D E_1\sim \a^4$.
% Thus, the energy splitting $\D E_1$ of the 1st excited state grows like $\a^2$ for small enough $\a$, large enough $L$.
% It turns out that $\D E_1\sim \a^4$ for $L=4$ due to the peculiarity of small system size, but the trend of $\D E_1\sim \a^2$ seems to hold for $L>4$. 

% The second point has been explained previously, so now we focus on the 3rd point.
% To explain the last point, we note that the 2nd excited states seem to come from those states with exactly 2 antiferromagnetic bonds such that they are maximally separated. For instance, for $L=6$, these states are ground states of the spin chain with bonds $(-1,1,1,-1,1,1)$ or cyclic permutations. There are $3=L/2$ such bond configurations. Moreover, since there are two ferromagnetic bonds between the antiferromagnetic ones, the ground state is 3-fold degenerate. Finally, note that each bond configuration corresponds to two different binary sequences. Thus, the number we get is $2\times 3\times L/2 =3N$ when $L=6$. This argument works for any $L\in 4\mathbb{Z}+2$, for which there would be an odd number of ferromagnetic bonds between the two antiferromagnetic ones.
% If $L\in 4\mathbb{Z}$, then would be an even number of ferromagnetic bonds between the two antiferromagnetic ones, so the ground state is unique for that bond configuration, and we get the number $2\times 1\times L/2 =L$.

% % We measure the ``gauge order parameter" $\langle \s^{45}_{j} \rangle$ in the lowest two energy levels, for $L=2,4,6$.
% % We found that the average gauge charge at each site is 0 for small $\a$.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Picture/DMRG PBC m=3 L=6 spectrum.png}
%     \caption{The lowest few energy gaps for $L=6$, $m=3$. When $\a=0$, the first excited state has $E_1-E_0\approx 0.965107$, and has degeneracy$=12$. All these 12 states are spin singlets. 4 pairs of the double singlet degeneracies are not lifted by the transverse term.}
%     \label{fig: DMRG PBC m=3 L=6 spectrum}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Picture/DMRG PBC m=3 L=10 spectrum.png}
%     \caption{The lowest few energy gaps for $L=10$, $m=3$.}
%     \label{fig: DMRG PBC m=3 L=10 spectrum}
% \end{figure}

% \begin{table}[H]
% \begin{center}
% \begin{tabular}{ |m{0.8cm}|| m{2cm} | m{2cm}| m{2cm}|}
%  \hline
%  $L$  & $\a_c$ & $E_{1,0}(\a_c,L)$ & $E_{2,0}(0,L)$ \\
%  \hline
%   4  & 0.869027 & 0.495954 & 1.0718 \\
%   6  & 0.8269(3) & 0.397(1) & 0.96511 \\
%   8  & 0.798(1)  &  0.336(1) & 0.897828(1) \\
%   10 & 0.775(1) & 0.295(2) & 0.854500(1)\\
%   12 & 0.758(2)  & 0.262(2)  & 0.824470(1)  \\
%   14 & 0.745(5)  & 0.236(1)  & 0.80244(1)   \\
%  \hline
% \end{tabular}
% \end{center}
% \caption{We used DMRG to solve the spectrum of $m=3$ TFGMM under PBC. We showed the critical values $\a_c$, the first excited energy gap at transition, and the energy gap at $\a=0$. The data for $L=4$ has a closed-form expression.}
% \end{table}

% From the data in the table above, we estimated the dependence of $\a_c$ on $L$ by a power law:
% \begin{align}
%     \ln\a_c=0.031(2)-0.1238(9)\ln L\,,
% \end{align}
% with $R^2=0.999747$.
% It seems to imply $\a_c\rightarrow 0$ in the thermodynamic limit.

\subsection{$m=5$}

For this special case, we write the Hamiltonian as
\begin{align}
    \hat{H}_5(\a,L)=\b\sum_{j=1}^{L}\sum_{\m=1}^{5}\g^\m_j\g^\m_{j+1}+\sqrt{1-\b^2}\sum_{j=1}^L\g^5_j\,,
\end{align}
where $-1\le \b \le 1$. This is because the sign of the hopping term matters.

There is no local symmetry.
When $|\b|=1$, there is $\mathrm{Spin}(5)$ global symmetry, generated by $\S^{\m\n}$ and $\S^{5\m}$.
When $|\b| < 1$, the global symmetry is $\mathrm{Spin}(4)$, generated by $\S^{\m\n}$.

For antiferromagnetic ($\b>0$) hopping terms, the ground state will become degenerate for some $\b$ with $|\b|<1$; for ferromagnetic ($\b<0$) hopping terms, the ground state is never degenerate if $|\b|<1$.

The 2-site problem has energy eigenstates of the form $\ket{E;s_+,m_+;s_-,m_-}$.
As in the case of $m=4$, these constitute 2 copies of spin singlets, triplets, and 4-vectors:
\begin{align}
   \text{singlets:}~~ \ket{\pm 2\sqrt{1+15\b^2}+2\b;0,0;0,0}\\
   M^-~\text{triplets:}~~   \ket{-2\sqrt{1-\b^2}+2\b;0,0;1,m_-}\\
    M^+~\text{triplets:}~~ \ket{2\sqrt{1-\b^2}+2\b;1,m_+;0,0}\\
    \text{4-vectors}~~\ket{(-2\pm 4)\b;\ha,m_+;\ha,m_-}\,.
\end{align}
As mentioned before, the ground state is degenerate for certain $\b$ away from $|\b|=0$ when $\b>0$. Indeed, one of the singlets
 is degenerate with one of the 4-vectors, having $E=-6$, when $\b=1$.
The expressions above show that the singlets have complicated dependence on both the hopping and the transverse terms; the triplets depend on those two terms in a simple (linear) manner; the 4-vectors depend only on the hopping term.

\begin{align}
     \hat{H}_{5,\text{eff}}=&L\left(-1+\b-\ha\b^2-\frac{1}{8}\b^4\right)\nonumber\\
     &+\b^2\left(1+\b-\ha \b^2\right)\sum_j \s^i_j\s^i_{j+1}\nonumber\\
     &+\frac{3\b^4}{4}\sum_j \s^i_{j}\s^i_{j+2}+\co(\b^5)\,.
\end{align}
Since it contains odd powers of $\b$, the $m=5$ TFGMM depends on the sign of $\b$.
The fluid-dimer transition corresponds to $(\a,\b)\approx (0.73,0.68)$ or $(\a,\b)\approx (0.91,-0.41)$.

 
\subsection{\label{subsec: gauge}Spatially local symmetries}
In $d+1$ spacetime dimensions, a local symmetry group is a symmetry group parameterized by arbitrary functions of the $d+1$ spacetime coordinates. 
A spatially local symmetry group is parameterized by arbitrary functions of only the $d$ spatial dimensions. 
The readers should be warned that it is common to equate a local symmetry with a gauge symmetry, but a spatially local symmetry need not be a gauge symmetry.
In some of our TFGMM, there are spatially local symmetries (s.l.s) such as $\mathrm{Spin}(3)=\mathrm{SU}(2)$ and $\mathrm{Spin}(2)=\mathrm{U}(1)$.
In the special case of $\a=0$, there could be extra symmetries, which will be explained in the coming sections.

In Table \ref{table: symmetries} below, we list all the spatially local and global symmetries for TFGMM at $\a>0$, excluding the global discrete symmetries already mentioned in the previous subsection.
In the column for spatially local symmetries, we only list the subgroup $\cg_j$ that acts on the local Hilbert space, because the full spatially local symmetry group is of the form $\cg=\bigotimes_j \cg_j$.

\begin{table}[H]
\begin{center}
\begin{tabular}{ |m{0.3cm}|| m{1.2cm}| m{1.8cm} | m{1.9cm}| m{2.4cm}|}
 \hline
 $m$  & s.l.s. $|\b|<1$ & s.l.s. generators & global sym. $|\b|<1$ & global sym. generators \\
 \hline
  1  & $\mathrm{Spin}(3)$ & $\s^{32},\s^{42},\s^{43}$ & $\mathbb{Z}_2\times\mathbb{Z}_2\times\mathbb{Z}_2$ & $(-1)^{L/2}\car_{\m\n}$, $\car_5$ \\
  2  & $\mathrm{Spin}(2)$ & $\s^{43}$  & $\mathrm{Spin}(2)$ & $\S^{12}$\\
  3  & $\emptyset$  &  & $\mathrm{Spin}(3)$ & $\S^{23},\S^{31},\S^{21}$ \\
  4 & $\emptyset$ &  & $\mathrm{Spin}(4)$  & $\S^{\m\n}$\\
  5 & $\emptyset$ &  & $\mathrm{Spin}(4)$  & $\S^{\m\n}$\\
 \hline
\end{tabular}
\end{center}
\caption{Global and spatially local symmetries of TFGMM for various values of $m$. We do not include the discrete global symmetries $T, P, \Q$ that all TFGMMs share.}
\label{table: symmetries}
\end{table}

We will study the cases of $m=1,2,3,4$ separately in the following sections. 
In section \ref{sec: m=1}, we show that the $m=1$ TFGMM is equivalent to a direct sum of $2^L$ copies of the transverse field Ising chain.
In section \ref{sec: m=2}, we show that the $m=2$ TFGMM is a direct sum of $2^L$ copies of frustrated Heisenberg spin-$\ha$ chains.
In section \ref{sec: m=3}, we show that the $m=3$ GMM is a direct sum of $2^L$ copies of $\mathrm{SO}(3)$-symmetric frustrated Heisenberg spin-$\ha$ chains when $\a=0$; for $\a>0$, it is more non-trivial.
In section \ref{sec: m=4}, we investigate the $m=4$ TFGMM which is much more complex than the cases of $m<4$; DMRG was used to calculate the spectrum and correlation functions for certain system sizes.
In section \ref{sec: m=5}, we briefly study the $m=5$ TFGMM, listing only some qualitative properties.


% \section{\label{append: Cl4 coherent states}Cl(4) coherent states }
% In theories with $\mathrm{O}(n)$ symmetry, it is natural to construct coherent states that are parameterized by the coordinates of $\mathbb{S}^{n-1}$.
% It turns out that, for $n>3$, we need at least another index to label these coherent states, i.e., we need vector coherent states instead of scalar coherent states.

% Now we define the $Cl(4)$ (vector) coherent states. 
% We require that the expectation value of $\g^\m$ with respect to the states labeled by spherical coordinates $(\f,\q,\varphi)$ is exactly a unit vector on $\mathbb{S}^3$ described by the coordinates. One way to realize this property is to define
% \begin{align}
%     |a;\f,\q,\varphi \rangle =U(\f,\q,\varphi)\ket{a}\,,~~a=1,2\\
%     \ket{1}=\frac{1}{\sqrt{2}}\begin{pmatrix}
%         1 \\ 0 \\ 1 \\ 0
%     \end{pmatrix}\,,~~\ket{2}=\frac{1}{\sqrt{2}}\begin{pmatrix}
%      0 \\ 1 \\ 0 \\ 1
%     \end{pmatrix}\\
%     U(\f,\q,\varphi)=\cos\frac{\varphi}{2}-i\sec\frac{\varphi}{2}V^\m\s^{\m 4}\\
%     V^1=\sin\f\sin\q\sin\varphi\,,~~V^2=\cos\f\sin\q\sin\varphi\,,\\
%     V^3=\cos\q\sin\varphi\,,~~V^4=\cos\varphi\,,
% \end{align}
% so that
% \begin{align}
%     \langle a;\f,\q,\varphi|\g^\m |b;\f,\q,\varphi \rangle=\d_{ab}V^\m\,,\label{eq: vectorial property of vcs}
% \end{align}
% where $\f\in [0,2\p)$ and $\q,\varphi \in [0,\p]$.
% $|a;\f,\q,\varphi \rangle$ differs from the more common $\mathrm{SU}(2)$ spin coherent states in that its specification requires a vector index $a=1,2$ in addition to the angular parameters. 

% We use coherent states when we want to ``dequantize" a quantum theory into a classical theory.
% To capture the spin-wave features of an $\mathrm{O}(n)$-symmetric quantum theory, the corresponding classical theory could contain vector fields transforming in the $\mathrm{O}(n)$ adjoint representation. 
% For the $\mathrm{O}(3)$-symmetric Heisenberg (anti)ferromagnetic chain, we use $\mathrm{SU}(2)$ spin coherent states satisfying a relation similar to Eq.(\ref{eq: vectorial property of vcs}) so that the classical theory has vector fields with the target space being $\mathbb{S}^2$.
% We claim that, in view of the $m=4$ GMM, the $Cl(4)$ vector coherent states are the most natural generalization of the $\mathrm{SU}(2)$ spin coherent states. 
% Just as the $\mathrm{O}(3)$-symmetric Heisenberg model contains the hopping term $\s^i_{j}\s^i_{j+1}\rightarrow \mathbf{V}(x_j)\cdot\mathbf{V}(x_{j+1})$, the $m=4$ GMM contains the hopping term $\g^\m_j\g^\m_{j+1}\rightarrow V^\m(x_j)V^\m(x_{j+1})$.
% Moreover, the spin coherent states $\ket{\f,\q}$ satisfies $\langle \f,\q |\s^i|\f,\q\rangle=V^i$, whereas the $Cl(4)$ vector coherent states satisfy Eq.(\ref{eq: vectorial property of vcs}).
% The biggest difference is that the $Cl(4)$ vector coherent states have a vector index $a$ that is absent in the spin coherent states. This is necessary: the coherent states must be invariant under the action of the subgroup $K=\mathrm{Spin}(3)=\mathrm{SU}(2)$ to preserve Eq.(\ref{eq: vectorial property of vcs}) for fixed angular parameters $(\f,\q,\varphi)$. This requirement implies that the space $\mathfrak{H}$ of all valid reference states from which we construct the coherent states must be $2$-dimensional. Hence, the resulting coherent states carry a label $a$ that can take $2$ values.

% It satisfies the resolution of unity in $\mathbb{C}^4$:
% \begin{align}
%     \frac{1}{\p^2}\int_{\mathbb{S}^3} d\O \sum_{a=1}^{2}|a;\f,\q,\varphi\rangle \langle a;\f,\q,\varphi |=1
% \end{align}
% where $d\O=d\varphi d\q d\f\, \sin\q \sin^2\varphi$.

% One downside of the vector coherent states is that they do not detect the transverse term.

\section{\label{sec: m=1} General $m$ TFGMM}
We define the $d=1$ transverse-field $\g$ matrix model (TFGMM) as the following families of Hamiltonians:
\begin{align}
    \hat{H}_m(\l)=\sum_{j=1}^{L}\left[\l\sum_{\m=1}^{m}\g^\m_j\g^\m_{j+1}+\sqrt{1-\l^2}\g^5_j\right]\,,\label{eq: TFGMM definition}
\end{align}
where $m=1,2,3,4,5$ and $-1\le \l \le 1$.  The $\g^5$ matrix is defined as $\g^5=-\g^1\g^2\g^3\g^4$.
When $\a=0$, we call $\hat{H}_{m}(\pm,0,L)$ as a $\g$ matrix model (GMM); for general $\a$, we call $\hat{H}_m(\pm,\a,L)$ as a TFGMM.
\subsection{$m=1$ and $m=2$}

It turns out that the $m<5$ TFGMM spectra are symmetrical under the $\mathbb{Z}_2\times\mathbb{Z}_2$ transformations, whereas the $m=5$ TFGMM spectrum is only invariant under $\car_{51}$ but not under $\car_{5}^{odd}$.
Hence, the sign of the transverse term doesn't matter; this fact justifies our usage of the transverse field parameter $\sqrt{1-\b^2}$.
Moreover, for $m<5$, we only need to consider the range $0\le \b\le 1$, whereas for $m=5$ we need the full range $-1\le \b \le 1$.

Let $\{b_j\}$ denote an arbitrary $L$-bit binary sequence. For each choice of such sequence, we can define a Hilbert subspace spanned by products of local states of the form $\bigotimes_{j}\ket{a_j,b_j}_j$, where $a_j=1,2$, and
\begin{align}
    \ket{1,+}=\begin{pmatrix}
        0 \\ 1 \\ 0 \\ 0
    \end{pmatrix}\,,~~\ket{2,+}=\begin{pmatrix}
        0 \\ 0 \\ 1 \\ 0
    \end{pmatrix}\,,\\
    \ket{1,-}=\begin{pmatrix}
        1 \\ 0 \\ 0 \\ 0
    \end{pmatrix}\,,~~\ket{2,-}=\begin{pmatrix}
        0 \\ 0 \\ 0 \\ 1
    \end{pmatrix}\,.
\end{align}
This basis allows us to split the total Hilbert space into $2^L$ many subspaces (one for each sequence $\{b_j\}$), each of dimension $2^L$. Then one can show that $\hat{H}_1$ and $\hat{H}_2$ act frustrated spin chains when restricted on these subspaces.

The $m=1$ TFGMM is equivalent to the direct sum of $2^L$ copies of the same Ising chain, each acting on only one Hilbert subspace associated with some $\{b_j\}$:
\begin{align}
     \hat{H}_{\text{Ising}}(\pm,\a,L)=\sum_{j}\left[\pm\sqrt{1-\a^2}\s^2_j \s^2_{j+1}+\a\s^3_j\right]\,.
\end{align}
Similarly, the $m=2$ TFGMM is the direct sum of $2^L$ copies of frustrated Heisenberg spin-$\ha$ chains:
\begin{align}
    \hat{H}_2(\pm,\a,L)&=\bigoplus_{\{b_j\}}\hat{H}_2[\{b_j\}]\,,\\
    \hat{H}_2[\{b_j\}]=&\pm\sqrt{1-\a^2}\sum_j (-1)^{b_j+b_{j+1}}\s^1_j\s^1_{j+1}\nonumber\\
    &\pm\sqrt{1-\a^2}\sum_j \s^2_j \s^2_{j+1}+\a\sum_j \s^3_j \,.\label{eq: m=2 spin chain}
\end{align}

As mentioned previously in \ref{subsec: gauge}, these two theories have spatially local symmetries. Our choice of basis $\ket{a,b_j}$ is compatible with these symmetries in that the symmetries do not mix states coming from subspaces defined by different sequences $\{b_j\}$.

\subsection{$m=3$}
When $|\b|=1$, there is a $\mathrm{U}(1)$ spatially local symmetry generated by $\s^{45}$. When $|\b| <1$, there is no local symmetry. There is an $\mathrm{SU}(2)$ global symmetry generated by $\S^{23},\S^{31},\S^{21}$. The spin quantum numbers corresponding to this global symmetry can be used to label the energy eigenstates. 

Now we solve the special case of $|\b|=1$, which does not involve any transverse term. 
We can choose the $\mathrm{U}(1)$ local gauge charge to be $\pm \ha$ at each site.
Each such choice is specified by the $L$-bit binary sequence $\{b_j\}$, where the spatially local symmetry charge at site $j$ is $(-1)^{b_j}\ha$.
At each site, the local Hilbert space corresponding to $b_j$ is spanned by the 2 eigenvectors of $(\s^{54})_j$ with eigenvalue $(-1)^{b_j}\ha$:
\begin{align}
    \ket{\pm,1}=\frac{1}{\sqrt{2}}\begin{pmatrix}
      \pm i \\ 0 \\ 1 \\ 0
    \end{pmatrix}\,,~~\ket{\pm,2}=\frac{1}{\sqrt{2}}\begin{pmatrix}
        0 \\ \pm i \\ 0 \\ 1
    \end{pmatrix}\,.
\end{align}
The global symmetry generators act on the local subspace at site $j$ by
\begin{align}
    \S^{ik}\ket{\pm,a}_j=-\frac{1}{2}\e^{ikl}(\s^l)_{ab}\ket{\pm, b}_j\,,
\end{align}
for $i,k,l\in\{1,2,3\}$.


Restricted to this local subspace, the $\g$ matrices that appear in $\hat{H}_3$ become 
\begin{align}
    (\g^i)_j\rightarrow (-1)^{b_j}(\s^i)_j ~~~~ i=1,2,3\,.
\end{align}
Thus, the theory is the direct sum
\begin{align}
    \hat{H}_3(\pm,0,L)=\bigoplus_{\{b_j\}}\hat{H}_3[\{b_j\}]\,,
\end{align}
where $\hat{H}_3[\{b_j\}]$ first projects to the Hilbert subspace corresponding to the sequence $\{b_j\}$, then act as
\begin{align}
    \hat{H}_3[\{b_j\}]=\pm\sum_{j}(-1)^{b_j+b_{j+1}}(\s^i)_{j}(\s^i)_{j+1}\,.
\end{align}

% A few observations for the $m=3$, $|\b|=1$ theory: 
% \begin{enumerate}
%     \item Each energy level has an even degeneracy. This is because $\hat{H}_3[\{b_j\}]=\hat{H}_3[\{b'_j\}]$ given that 
%     \begin{align}
%         b_j=b'_j+1 ~~(\text{mod} 2)~~~\forall j=1,\cdots,L\,.
%     \end{align}
%     \item The ground state energy of the $m=3$ GMM is exactly the ground state energy of the antiferromagnetic Heisenberg spin-$\ha$ chain. Such a spin chain is described by $b_j=constant$ for all $j=1,2,\cdots, L$ in our Hamiltonian. Since the constant can only take two values (either 0 or 1), the ground state is doubly degenerate, consistent with the previous point.
%     \item For any integer $L>2$ and any choice of the $L$-bit binary sequence $\{b_j\}$, there are an even number of ferromagnetic bonds (FB) in $\hat{H}_3[\{b_j\}]$, i.e. bonds that have coefficient $-1$.
%     \item Generally, the less frustration (number of domain walls) a spin chain has, the lower its ground state energy. 
%     \item For those Hamiltonians with exactly two ferromagnetic bonds (FB), if there are an even number of antiferromagnetic bonds (AFB) between the FBs, then the ground state is 3-fold degenerate; if there are an odd number of AFBs between the two FBs, then the ground state is unique.
%     \item After the antiferromagnetic Heisenberg chain, the Hamiltonians $\hat{H}_3[\{b_j\}]$ with the next lowest ground state have exactly two ferromagnetic bonds that are separated from each other by exactly one AFB.
% \end{enumerate}
% For instance, for $L=4$, the first excited states are ground states for the spin chain with bond coefficients $(1,-1,1,-1)$ and $(-1,1,-1,1)$. Therefore, the first excited energy level has a degeneracy of $2\times 2=4$.
% For $L=6$, the first excited states are ground states for the spin chain with bond coefficients $(-1,1,-1,1,1,1)$, $(1,-1,1,-1,1,1)$, $(1,1,-1,1,-1,1)$, $(1,1,1,-1,1,-1)$, $(-1,1,1,1,-1,1)$, and $(1,-1,1,1,1,-1)$. Therefore, the first excited energy level has a degeneracy of $2\times 6=12$.
% If this argument is true in general, then we expect the first excited state to be $2N$-fold degenerate for any even $L>2$. Indeed, this is what we observe for small system sizes: it has been verified up to $L=8$.

% The method explained in this subsection do not work for $m=4$, since $\g^4$ mixes the $\pm$ subspaces:
% \begin{align}
%     \g^4\ket{\pm,a}=\pm i \ket{\mp,a}\,.
% \end{align}

% Finally, we note that there is a way to understand why the sign of the hopping term for the $m=3$ TFGMM doesn't matter. 
% We have just seen that the Hamiltonian is the direct sum of all possible $\mathrm{O}(3)$-symmetric Heisenberg spin-$\ha$ chains, including the antiferromagnetic chain and the ferromagnetic chain.
% Multiplying the hopping terms by a sign may map one spin chain to another, but the new Hamiltonian is still the same direct sum of all possible Heisenberg spin chains.

The $\a\ne 0$ case is much trickier than the $\a=0$ case.
The local invariant subspace for all of $\g^1_j,\g^2_j,\g^3_j,\g^5_j$ is simply the 4-dimensional local Hilbert space because
\begin{align}
     \g^5\ket{\pm,a}=- \ket{\mp,a}\,,
\end{align}
so we cannot decompose $\hat{H}_3(\b,L)$ into a direct sum.
Moreover, there is no spatially local symmetry.

% We show that there is an interesting duality: there is an equivalent theory in which the on-site interaction term corresponds to the TFGMM's hopping term, and the hopping term corresponds to the TFGMM's on-site interaction terms. 
% Consider an array of $2^L$ many Heisenberg spin-$\ha$ chains, where each chain is seen as a ``site". Each such site has a unique site index $I$, ranging from $0$ to $2^L-1$. We choose to represent $I$ in binary digits: $I=0,1,10,11,100$, etc. In other words, the set of all index $I$ is isomorphic to the set of all $L$-bit binary sequences $\{b_j\}$. 
% Moreover, we say $I'$ is a neighbor of $I\sim\{b_j\}$ whenever $I'-I\in (-1)^{b_k} 2^{k-1}$ for some positive integer $k$.
% Thus, each site has exactly $L$ neighbors.
% Now we specify that the spin chain at site $\{b_j\}$ is exactly $\hat{H}_{3}[\{b_j\}]$ as described in the previous subsection.
% Thus, the hopping terms $\sum_{\m=1}^{3}\g^\m_j\g^\m_{j+1}$ from the original Hamiltonian $\hat{H}_3$ now correspond to on-site terms in the new perspective.
% Similarly, the on-site interaction term $\g^5_j $ from the original Hamiltonian now becomes a hopping term. 
% At the site $I\sim \{b_j\}$, the local Hilbert space is $2^L$-dimensional and is spanned by tensor product states of the form $\ket{I;\{a_j\}}$, where $a_j=1,2$. Then $\g^5_k$ acts by
% \begin{align}
%     \g^5_k\ket{I;\{a_j\}}=-\ket{I+(-1)^{b_k}2^{k-1};\{a_j\}}\,.
% \end{align}
% By our definition of neighboring spin chains, the interaction term $\g^5_k$ which is on-site in the original Hamiltonian can now be seen as a nearest-neighbor hopping term.
% In fact, it is like the translation operators in an $L$-dimensional space.
% There are important differences between these two perspectives. In the original view, the Hilbert space is a tensor product of local Hilbert spaces, whereas now the Hilbert space is a direct sum of local Hilbert spaces. Moreover, originally the on-site terms are position-independent, but now the on-site terms are position-dependent. 
% We will not go further with this analogy.




he $\g^5$ matrix is defined as $\g^5=-\g^1\g^2\g^3\g^4$.
When $\a=0$, we call $\hat{H}_{m}(\pm,0,L)$ as a $\g$ matrix model (GMM); for general $\a$, we call $\hat{H}_m(\pm,\a,L)$ as a TFGMM.
\subsection{$m=1$ and $m=2$}

It turns out that the $m<5$ TFGMM spectra are symmetrical under the $\mathbb{Z}_2\times\mathbb{Z}_2$ transformations, whereas the $m=5$ TFGMM spectrum is only invariant under $\car_{51}$ but not under $\car_{5}^{odd}$.
Hence, the sign of the transverse term doesn't matter; this fact justifies our usage of the transverse field parameter $\sqrt{1-\b^2}$.
Moreover, for $m<5$, we only need to consider the range $0\le \b\le 1$, whereas for $m=5$ we need the full range $-1\le \b \le 1$.

Let $\{b_j\}$ denote an arbitrary $L$-bit binary sequence. For each choice of such sequence, we can define a Hilbert subspace spanned by products of local states of the form $\bigotimes_{j}\ket{a_j,b_j}_j$, where $a_j=1,2$, and
\begin{align}
    \ket{1,+}=\begin{pmatrix}
        0 \\ 1 \\ 0 \\ 0
    \end{pmatrix}\,,~~\ket{2,+}=\begin{pmatrix}
        0 \\ 0 \\ 1 \\ 0
    \end{pmatrix}\,,\\
    \ket{1,-}=\begin{pmatrix}
        1 \\ 0 \\ 0 \\ 0
    \end{pmatrix}\,,~~\ket{2,-}=\begin{pmatrix}
        0 \\ 0 \\ 0 \\ 1
    \end{pmatrix}\,.
\end{align}
This basis allows us to split the total Hilbert space into $2^L$ many subspaces (one for each sequence $\{b_j\}$), each of dimension $2^L$. Then one can show that $\hat{H}_1$ and $\hat{H}_2$ act frustrated spin chains when restricted on these subspaces.

The $m=1$ TFGMM is equivalent to the direct sum of $2^L$ copies of the same Ising chain, each acting on only one Hilbert subspace associated with some $\{b_j\}$:
\begin{align}
     \hat{H}_{\text{Ising}}(\pm,\a,L)=\sum_{j}\left[\pm\sqrt{1-\a^2}\s^2_j \s^2_{j+1}+\a\s^3_j\right]\,.
\end{align}
Similarly, the $m=2$ TFGMM is the direct sum of $2^L$ copies of frustrated Heisenberg spin-$\ha$ chains:
\begin{align}
    \hat{H}_2(\pm,\a,L)&=\bigoplus_{\{b_j\}}\hat{H}_2[\{b_j\}]\,,\\
    \hat{H}_2[\{b_j\}]=&\pm\sqrt{1-\a^2}\sum_j (-1)^{b_j+b_{j+1}}\s^1_j\s^1_{j+1}\nonumber\\
    &\pm\sqrt{1-\a^2}\sum_j \s^2_j \s^2_{j+1}+\a\sum_j \s^3_j \,.\label{eq: m=2 spin chain}
\end{align}

As mentioned previously in \ref{subsec: gauge}, these two theories have spatially local symmetries. Our choice of basis $\ket{a,b_j}$ is compatible with these symmetries in that the symmetries do not mix states coming from subspaces defined by different sequences $\{b_j\}$.

\subsection{$m=5$}

For this special case, we write the Hamiltonian as
\begin{align}
    \hat{H}_5(\a,L)=\b\sum_{j=1}^{L}\sum_{\m=1}^{5}\g^\m_j\g^\m_{j+1}+\sqrt{1-\b^2}\sum_{j=1}^L\g^5_j\,,
\end{align}
where $-1\le \b \le 1$. This is because the sign of the hopping term matters.

There is no local symmetry.
When $|\b|=1$, there is $\mathrm{Spin}(5)$ global symmetry, generated by $\S^{\m\n}$ and $\S^{5\m}$.
When $|\b| < 1$, the global symmetry is $\mathrm{Spin}(4)$, generated by $\S^{\m\n}$.

For antiferromagnetic ($\b>0$) hopping terms, the ground state will become degenerate for some $\b$ with $|\b|<1$; for ferromagnetic ($\b<0$) hopping terms, the ground state is never degenerate if $|\b|<1$.

The 2-site problem has energy eigenstates of the form $\ket{E;s_+,m_+;s_-,m_-}$.
As in the case of $m=4$, these constitute 2 copies of spin singlets, triplets, and 4-vectors:
\begin{align}
   \text{singlets:}~~ \ket{\pm 2\sqrt{1+15\b^2}+2\b;0,0;0,0}\\
   M^-~\text{triplets:}~~   \ket{-2\sqrt{1-\b^2}+2\b;0,0;1,m_-}\\
    M^+~\text{triplets:}~~ \ket{2\sqrt{1-\b^2}+2\b;1,m_+;0,0}\\
    \text{4-vectors}~~\ket{(-2\pm 4)\b;\ha,m_+;\ha,m_-}\,.
\end{align}
As mentioned before, the ground state is degenerate for certain $\b$ away from $|\b|=0$ when $\b>0$. Indeed, one of the singlets
 is degenerate with one of the 4-vectors, having $E=-6$, when $\b=1$.
The expressions above show that the singlets have complicated dependence on both the hopping and the transverse terms; the triplets depend on those two terms in a simple (linear) manner; the 4-vectors depend only on the hopping term.

\begin{align}
     \hat{H}_{5,\text{eff}}=&L\left(-1+\b-\ha\b^2-\frac{1}{8}\b^4\right)\nonumber\\
     &+\b^2\left(1+\b-\ha \b^2\right)\sum_j \s^i_j\s^i_{j+1}\nonumber\\
     &+\frac{3\b^4}{4}\sum_j \s^i_{j}\s^i_{j+2}+\co(\b^5)\,.
\end{align}
Since it contains odd powers of $\b$, the $m=5$ TFGMM depends on the sign of $\b$.
The fluid-dimer transition corresponds to $(\a,\b)\approx (0.73,0.68)$ or $(\a,\b)\approx (0.91,-0.41)$.

 
\subsection{\label{subsec: gauge}Spatially local symmetries}
In $d+1$ spacetime dimensions, a local symmetry group is a symmetry group parameterized by arbitrary functions of the $d+1$ spacetime coordinates. 
A spatially local symmetry group is parameterized by arbitrary functions of only the $d$ spatial dimensions. 
The readers should be warned that it is common to equate a local symmetry with a gauge symmetry, but a spatially local symmetry need not be a gauge symmetry.
In some of our TFGMM, there are spatially local symmetries (s.l.s) such as $\mathrm{Spin}(3)=\mathrm{SU}(2)$ and $\mathrm{Spin}(2)=\mathrm{U}(1)$.
In the special case of $\a=0$, there could be extra symmetries, which will be explained in the coming sections.

In Table \ref{table: symmetries} below, we list all the spatially local and global symmetries for TFGMM at $\a>0$, excluding the global discrete symmetries already mentioned in the previous subsection.
In the column for spatially local symmetries, we only list the subgroup $\cg_j$ that acts on the local Hilbert space, because the full spatially local symmetry group is of the form $\cg=\bigotimes_j \cg_j$.

\begin{table}[H]
\begin{center}
\begin{tabular}{ |m{0.3cm}|| m{1.2cm}| m{1.8cm} | m{1.9cm}| m{2.4cm}|}
 \hline
 $m$  & s.l.s. $|\b|<1$ & s.l.s. generators & global sym. $|\b|<1$ & global sym. generators \\
 \hline
  1  & $\mathrm{Spin}(3)$ & $\s^{32},\s^{42},\s^{43}$ & $\mathbb{Z}_2\times\mathbb{Z}_2\times\mathbb{Z}_2$ & $(-1)^{L/2}\car_{\m\n}$, $\car_5$ \\
  2  & $\mathrm{Spin}(2)$ & $\s^{43}$  & $\mathrm{Spin}(2)$ & $\S^{12}$\\
  3  & $\emptyset$  &  & $\mathrm{Spin}(3)$ & $\S^{23},\S^{31},\S^{21}$ \\
  4 & $\emptyset$ &  & $\mathrm{Spin}(4)$  & $\S^{\m\n}$\\
  5 & $\emptyset$ &  & $\mathrm{Spin}(4)$  & $\S^{\m\n}$\\
 \hline
\end{tabular}
\end{center}
\caption{Global and spatially local symmetries of TFGMM for various values of $m$. We do not include the discrete global symmetries $T, P, \Q$ that all TFGMMs share.}
\label{table: symmetries}
\end{table}

We will study the cases of $m=1,2,3,4$ separately in the following sections. 
In section \ref{sec: m=1}, we show that the $m=1$ TFGMM is equivalent to a direct sum of $2^L$ copies of the transverse field Ising chain.
In section \ref{sec: m=2}, we show that the $m=2$ TFGMM is a direct sum of $2^L$ copies of frustrated Heisenberg spin-$\ha$ chains.
In section \ref{sec: m=3}, we show that the $m=3$ GMM is a direct sum of $2^L$ copies of $\mathrm{SO}(3)$-symmetric frustrated Heisenberg spin-$\ha$ chains when $\a=0$; for $\a>0$, it is more non-trivial.
In section \ref{sec: m=4}, we investigate the $m=4$ TFGMM which is much more complex than the cases of $m<4$; DMRG was used to calculate the spectrum and correlation functions for certain system sizes.
In section \ref{sec: m=5}, we briefly study the $m=5$ TFGMM, listing only some qualitative properties.

Now we solve the special case of $|\b|=1$, which does not involve any transverse term. 
We can choose the $\mathrm{U}(1)$ local gauge charge to be $\pm \ha$ at each site.
Each such choice is specified by the $L$-bit binary sequence $\{b_j\}$, where the spatially local symmetry charge at site $j$ is $(-1)^{b_j}\ha$.
At each site, the local Hilbert space corresponding to $b_j$ is spanned by the 2 eigenvectors of $(\s^{54})_j$ with eigenvalue $(-1)^{b_j}\ha$:
\begin{align}
    \ket{\pm,1}=\frac{1}{\sqrt{2}}\begin{pmatrix}
      \pm i \\ 0 \\ 1 \\ 0
    \end{pmatrix}\,,~~\ket{\pm,2}=\frac{1}{\sqrt{2}}\begin{pmatrix}
        0 \\ \pm i \\ 0 \\ 1
    \end{pmatrix}\,.
\end{align}
The global symmetry generators act on the local subspace at site $j$ by
\begin{align}
    \S^{ik}\ket{\pm,a}_j=-\frac{1}{2}\e^{ikl}(\s^l)_{ab}\ket{\pm, b}_j\,,
\end{align}
for $i,k,l\in\{1,2,3\}$.


Restricted to this local subspace, the $\g$ matrices that appear in $\hat{H}_3$ become 
\begin{align}
    (\g^i)_j\rightarrow (-1)^{b_j}(\s^i)_j ~~~~ i=1,2,3\,.
\end{align}
Thus, the theory is the direct sum
\begin{align}
    \hat{H}_3(\pm,0,L)=\bigoplus_{\{b_j\}}\hat{H}_3[\{b_j\}]\,,
\end{align}
where $\hat{H}_3[\{b_j\}]$ first projects to the Hilbert subspace corresponding to the sequence $\{b_j\}$, then act as
\begin{align}
    \hat{H}_3[\{b_j\}]=\pm\sum_{j}(-1)^{b_j+b_{j+1}}(\s^i)_{j}(\s^i)_{j+1}\,.
\end{align}

The $\a\ne 0$ case is much trickier than the $\a=0$ case.
The local invariant subspace for all of $\g^1_j,\g^2_j,\g^3_j,\g^5_j$ is simply the 4-dimensional local Hilbert space because
\begin{align}
     \g^5\ket{\pm,a}=- \ket{\mp,a}\,,
\end{align}
so we cannot decompose $\hat{H}_3(\b,L)$ into a direct sum.
Moreover, there is no spatially local symmetry.

The 2-site problem has energy eigenstates of the form $\ket{E,s,m_s}$, which are either spin singlets or triplets. The triplets ($s=1$) have energies  $E=\pm 2$ and $E=\pm 2\sqrt{1-\a^2}$. 
The spin singlets ($s=0$) have energies $E=\pm 6\sqrt{1-\a^2}$ and $E=\pm 2\sqrt{9-8\a^2}$. 


The effective Hamiltonian acting on the nearly $2^L$-fold degenerate ground state at the regime of $\a=\sqrt{1-\e^2}$ where $0\le \e \ll 1$ (in the fermionic perspective, this is at half-filling) is
\begin{align}
    \hat{H}_{3,\text{eff}}=&L\left(-1-\frac{1}{4}\e^2+\frac{11}{64}\e^4\right)\nonumber\\
    &+\e^2\left(\ha-\frac{7}{16}\e^2\right)\sum_{j}\s^i_j\s^i_{j+1}\nonumber\\
    &+\frac{\e^4}{4}\sum_{j}\s^i_j\s^i_{j+2}+\co(\e^5)\,.
\end{align}
which is an antiferromagnetic spin-$\ha$ $J_1-J_2$ model up to the 4th order.
Note that this expression is valid only for $L>4$. For $L<4$, it is slightly different, but since these simple cases can be studied exactly without using any perturbation theory, we don't bother to discuss them.

two the dangling sites need to be connected as a singlets are connected via 


subspaces $\cg_L$ for $H^o_L$. For even $L\ge 6$, the ground state subspaces $\cg'_L$ for $H^p_L$ are two-fold degenerate. 

get either the $L$-site open-boundary Majumdar-Ghosh GMM $H^o_L$ or the periodic Majumdar-Ghosh GMM $H^p_L$, defined by
\begin{align}
    H^o_L=\sum_{j=1}^{L-2}K_j\,,~~H^p_L=\sum_{j=1}^{L}K_j\,,
\end{align}
where 
\begin{align}
    K_j=\sum_{\m=1}^{4}(\g^\m_{j}+\g^\m_{j+1}+\g^\m_{j+2})^2-4\,.
\end{align}
$K_j$ is a non-negative Hermitian operator. 



Denote the Spin(4) singlet ground state of the 2-site Hamiltonian $\sum_{\m=1}^{4}\g_i^\m \g_j^\m$ as $\ket{i;j}$. 

We denote the Dirac representation at site $i$ as $\mathrm{Dirac}_{i}$, i.e. it is the local Hilbert space $\mathbb{C}^4$ at site $i$ that transforms as $(\ha,0)\oplus (0,\ha)$ under the generators $\s^{\m\n}_i$. for odd $L=2k+1$, define the Hilbert subspaces $V_{L}, V'_{L}$ by
\begin{align}
    V_{2k+1}=\ket{1;2}\otimes \cdots \otimes \ket{2k-1;2k}\otimes \mathrm{Dirac}_{2k+1}\,,\\
    V'_{2k+1}=\mathrm{Dirac}_{1}\otimes \ket{2;3}\otimes \cdots \otimes \ket{2k;2k+1}\,.
\end{align}
For even $L=2k$, define the Hilbert subspace $W_{L}$ by
\begin{align}
  W_{2k}&=\mathrm{Dirac}_1\otimes \bigotimes_{p=1}^{k-1} \ket{2p;2p+1} \otimes \mathrm{Dirac}_{2k} \,.
\end{align}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{Picture/G4 subspace.pdf}
    \caption{The figure shows $\cg_4=W_4\oplus \mathrm{span}\{\ket{1;2}\otimes\ket{3;4},\ket{1;3}\otimes\ket{2;4}\}$.}
    \label{fig: G4}
\end{figure}



The NNN GMM is in the gapped dimerized phase for the whole range $0\le J_2/J_1\le 0.5$, as can be seen in Fig.\ref{fig: NNN GMM gap}.


% We focus on the case where $J_1, J_2\ge 0$, so we can set $J_2=\a$ and $J_1=\sqrt{1-\a^2}$. Using DMRG, one can easily show that the model at any $L$ always has a degenerate GS at the \textit{Majumdar-Ghosh point} where $\a=\frac{1}{\sqrt{5}}$ (or equivalently $J_2/J_1=\ha$).
% More specifically,
% \begin{itemize}
%     \item For odd $L>3$, the GS is always 8-fold degenerate for all $\a$.
%     \item When $L=4$, this GS is 3-fold degenerate at $\frac{J_2}{J_1}=\ha$.
%     \item For even $L>4$, the GS is exactly 2-fold degenerate at $\frac{J_2}{J_1}=\ha$.
%     \item All the degenerate ground states are spin singlets.
% \end{itemize}
% The GS energy density at the exactly dimerized point is exactly $E_0/L=-\frac{4}{\sqrt{5}}$ even for finite even $L$, which has been verified using DMRG for $L=4,6,8,10,12,...,20$ up to accuracy of order $10^{-15}$.
% On the other hand, when $L$ is odd, the GS energy density depends on $L$.

% Let us try to explain the exact dimerization for even $L$. We start by rewriting the $J_1$-$J_2$ GMM at the Majumdar-Ghosh point:
% \begin{align}
%     \hat{H}&=\frac{1}{\sqrt{5}}\sum_{j=1}^{L}\sum_{\m=1}^{4}\left(2\g^\m_j\g^\m_{j+1}+\g^\m_j\g^\m_{j+2}\right)\\
%     &=\frac{1}{2\sqrt{5}}\sum_{j=1}^{L}\sum_{\m=1}^{4}\left(\g^\m_j+\g^\m_{j-1}+\g^\m_{j+1}\right)^2-\frac{6L}{\sqrt{5}}\,.
% \end{align}
% We note that 4 is the minimum eigenvalue of the Hermitian operator 
% \begin{align}
%      K_j:=\sum_{\m=1}^{4}\left(\g^\m_j+\g^\m_{j-1}+\g^\m_{j+1}\right)^2
% \end{align}
% so we know the GS energy density $E_0/L=-4/\sqrt{5}$ can be achieved if and only if there is a state $\ket{\j}$ satisfying the 3-site relation
% \begin{align}
%     K_j\ket{\j}=4\ket{\j}
% \end{align}
% for all site $j$.
% If $L=3$, then the equation above has exactly 12 solutions, corresponding to 
% \begin{align}
%    \text{Type I}: [1;2]\otimes e^\m_{3}\,,\\
%    \text{Type II}: [1;3]\otimes e^\m_{2}\,,\\
%    \text{Type III}: e^\m_1\otimes [2;3]\,, 
% \end{align}
% where $e^\m_k$ is the $\m$-th unit vector in the site-$k$ local Hilbert space, and $[i;j]$ is the GS of the 2-site GMM $\sum_{\m=1}^{4}\g^\m_i\g^\m_j$.
% Now consider a bigger lattice where $L>3$, and start looking at the Hilbert subspace $\ch_{1,2,3}$ based on the sublattice consisting of sites $1,2,3$. The GS $\ket{\j}$ of the full system must have components whose projection to this sublattice is either of Type I, II, or III (can be two types at the same time) so that $K_{2}\ket{\j}=4\ket{\j}$.
% If it is Type I, then the unpaired spin in site 3 must form a singlet with site 4 so that $K_{3}\ket{\j}=4\ket{\j}$, i.e. it is of Type III in $\ch_{2,3,4}$. This pattern then repeats itself. If $L$ is even, then this choice gives us a completely dimerized state. The argument is the same for the subsystem $\ch_{1,2,3}$ having a GS in Type III, giving us the second of the dimerized state if $L$ is even. 
% What if we started with Type II?
% If we start with Type II in $\ch_{1,2,3}$, then to get the lowest possible 2-bond energy it must also be of Type II in $\ch_{2,3,4}$; but then $G_4$ will not be acting on singlet bonds unless $L=4$, which explains why $L=4$ has a trimerized GS.
% If $L>4$ this will lead to at least one frustration, so this Type II cannot be part of the GS for even $L>4$. 
% To conclude, we have shown that $L=4$ has a trimerized ground state, whereas larger even $L$ has a dimerized ground state. 

